A (More) Realistic Evaluation Setup for Generalisation of Community Models on Malicious Content Detection

Community models for malicious content detection, which take into account the context from a social graph alongside the content itself, have shown remarkable performance on benchmark datasets. Yet, misinformation and hate speech continue to propagate on social media networks. This mismatch can be partially attributed to the limitations of current evaluation setups that neglect the rapid evolution of online content and the underlying social graph. In this paper, we propose a novel evaluation setup for model generalisation based on our few-shot subgraph sampling approach. This setup tests for generalisation through few labelled examples in local explorations of a larger graph, emulating more realistic application settings. We show this to be a challenging inductive setup, wherein strong performance on the training graph is not indicative of performance on unseen tasks, domains, or graph structures. Lastly, we show that graph meta-learners trained with our proposed few-shot subgraph sampling outperform standard community models in the inductive setup. We make our code publicly available.

==> tables/ablation_experiment.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[t]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}[2]{*}{\textbf{k}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{CoAID}} & \multicolumn{2}{c}{\textbf{TwitterHateSpeech}} \\
        & & Trained & Reset & Trained & Reset \\
        \midrule
        \multirow{2}[2]{*}{4}  
        & MAML & \makecell{\small{0.1195}\\[-5pt] \footnotesize{(0.1177, 0.1214)}} & \makecell{\small{0}\\[-5pt] \footnotesize{(0, 0)}} & \makecell{\small{0.0543}\\[-5pt] \footnotesize{(0.0507, 0.0579)}} & \makecell{\small{0.0726}\\[-5pt] \footnotesize{(0.0687, 0.0765)}} \\[-3pt]
        & ProtoMAML & \makecell{\small{0.1383}\\[-5pt] \footnotesize{(0.1343, 0.1422)}} & \makecell{\small{0.1191}\\[-5pt] \footnotesize{(0.1114, 0.1268)}} & \makecell{\small{0.0607}\\[-5pt] \footnotesize{(0.0565, 0.0648)}} & \makecell{\small{0.0767}\\[-5pt] \footnotesize{(0.0729, 0.0806)}} \\[-3pt]
        \midrule
        \multirow{2}[2]{*}{8} 
        & MAML & \makecell{\small{0.1312}\\[-5pt] \footnotesize{(0.1297, 0.1326)}} & \makecell{\small{0}\\[-5pt] \footnotesize{(0, 0)}} & \makecell{\small{0.0515}\\[-5pt] \footnotesize{(0.0483, 0.0546)}} & \makecell{\small{0.0811}\\[-5pt] \footnotesize{(0.0777, 0.0846)}} \\[-3pt]
        & ProtoMAML & \makecell{\small{0.1709}\\[-5pt] \footnotesize{(0.1685, 0.1733)}} & \makecell{\small{0.1398}\\[-5pt] \footnotesize{(0.1361, 0.1434)}} & \makecell{\small{0.0699}\\[-5pt] \footnotesize{(0.0657, 0.074)}} & \makecell{\small{0.0868}\\[-5pt] \footnotesize{(0.0832, 0.0904)}} \\[-3pt]
        \midrule
        \multirow{2}[2]{*}{12} 
        & MAML & \makecell{\small{0.1281}\\[-5pt] \footnotesize{(0.1267, 0.1295)}} & \makecell{\small{0}\\[-5pt] \footnotesize{(0, 0)}} & \makecell{\small{0.0791}\\[-5pt] \footnotesize{(0.0757, 0.0824)}} & \makecell{\small{0.0969}\\[-5pt] \footnotesize{(0.0938, 0.1001)}} \\[-3pt]
        & ProtoMAML & \makecell{\small{0.1689}\\[-5pt] \footnotesize{(0.1669, 0.1708)}} & \makecell{\small{0.1304}\\[-5pt] \footnotesize{(0.1262, 0.1347)}} & \makecell{\small{0.1109}\\[-5pt] \footnotesize{(0.1066, 0.1152)}} & \makecell{\small{0.1025}\\[-5pt] \footnotesize{(0.0997, 0.1053)}} \\[-3pt]
        \midrule
        \multirow{2}[2]{*}{16} 
        & MAML & \makecell{\small{0.1234}\\[-5pt] \footnotesize{(0.1221, 0.1247)}} & \makecell{\small{0}\\[-5pt] \footnotesize{(0, 0)}} & \makecell{\small{0.0811}\\[-5pt] \footnotesize{(0.0778, 0.0844)}} & \makecell{\small{0.0980}\\[-5pt] \footnotesize{(0.095, 0.1009)}} \\[-3pt]
        & ProtoMAML & \makecell{\small{0.1646}\\[-5pt] \footnotesize{(0.1631, 0.1662)}} & \makecell{\small{0.1212}\\[-5pt] \footnotesize{(0.1179, 0.1245)}} & \makecell{\small{0.1354}\\[-5pt] \footnotesize{(0.1303, 0.1404)}} & \makecell{\small{0.1052}\\[-5pt] \footnotesize{(0.1025, 0.1078)}} \\[-3pt]
        \bottomrule
    \end{tabular}
    %}
    \caption{Comparison of trained and reset models in terms of MCC. In each row section, top row corresponds to \textsc{maml-rh}, bottom to \textsc{protomaml}. Brackets give the 90\% confidence interval.}
    \label{tab:reset_comparison}
\end{table*}


==> tables/coaid_mlp_ubs_transfer.tex <==
% Table generated by Excel2LaTeX from sheet 'Transfer CoAID - Low Adapt'
\begin{table*}[h]
    \centering
    \begin{tabular}{clccccc}
        \toprule
        \multirow{2}[4]{*}{\textbf{k}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Real}} & \multicolumn{2}{c}{\textbf{Fake}} & \textbf{Aggregate} \\
        \cmidrule(l{4pt}r{4pt}){3-4} \cmidrule(l{4pt}r{4pt}){5-6} \cmidrule(l{4pt}r{4pt}){7-7}
        &       & \textbf{F1} & \textbf{AUPR} & \textbf{F1} & \textbf{AUPR} & \textbf{MCC} \\
        \midrule
        \multirow{3}[2]{*}{4}
            & Subgraphs & \makecell{\small{0.6615}\\[-5pt] \footnotesize{(0.6534, 0.6695)}} & \makecell{\small{0.9631}\\[-5pt] \footnotesize{(0.9624, 0.9639)}} & \makecell{\small{0.1394}\\[-5pt] \footnotesize{(0.1376, 0.1412)}} & \makecell{\small{0.1042}\\[-5pt] \footnotesize{(0.1025, 0.1058)}} & \makecell{\small{0.0879}\\[-5pt] \footnotesize{(0.0848, 0.091)}} \\
            & MAML  & \makecell{\small{0.685}\\[-5pt] \footnotesize{(0.676, 0.694)}} & \makecell{\small{0.9537}\\[-5pt] \footnotesize{(0.9531, 0.9544)}} & \makecell{\small{0.1238}\\[-5pt] \footnotesize{(0.1219, 0.1257)}} & \makecell{\small{0.0762}\\[-5pt] \footnotesize{(0.0752, 0.0773)}} & \makecell{\small{0.05}\\[-5pt] \footnotesize{(0.0466, 0.0533)}} \\
            & ProtoMAML & \makecell{\small{0.6519}\\[-5pt] \footnotesize{(0.6449, 0.6589)}} & \makecell{\small{0.9721}\\[-5pt] \footnotesize{(0.9715, 0.9726)}} & \makecell{\small{0.1528}\\[-5pt] \footnotesize{(0.151, 0.1547)}} & \makecell{\small{0.1361}\\[-5pt] \footnotesize{(0.1333, 0.1389)}} & \makecell{\small{0.1204}\\[-5pt] \footnotesize{(0.1172, 0.1236)}} \\
        \midrule
        \multirow{3}[2]{*}{8}
            & Subgraphs & \makecell{\small{0.6781}\\[-5pt] \footnotesize{(0.6704, 0.6858)}} & \makecell{\small{0.9695}\\[-5pt] \footnotesize{(0.9689, 0.97)}} & \makecell{\small{0.1462}\\[-5pt] \footnotesize{(0.1444, 0.148)}} & \makecell{\small{0.109}\\[-5pt] \footnotesize{(0.1074, 0.1106)}} & \makecell{\small{0.1112}\\[-5pt] \footnotesize{(0.1082, 0.1142)}} \\
            & MAML  & \makecell{\small{0.7174}\\[-5pt] \footnotesize{(0.7089, 0.7258)}} & \makecell{\small{0.9622}\\[-5pt] \footnotesize{(0.9616, 0.9628)}} & \makecell{\small{0.1271}\\[-5pt] \footnotesize{(0.1256, 0.1287)}} & \makecell{\small{0.0791}\\[-5pt] \footnotesize{(0.0782, 0.0801)}} & \makecell{\small{0.0724}\\[-5pt] \footnotesize{(0.0694, 0.0753)}} \\
            & ProtoMAML & \makecell{\small{0.6929}\\[-5pt] \footnotesize{(0.6876, 0.6982)}} & \makecell{\small{0.9778}\\[-5pt] \footnotesize{(0.9774, 0.9782)}} & \makecell{\small{0.1567}\\[-5pt] \footnotesize{(0.1552, 0.1583)}} & \makecell{\small{0.1384}\\[-5pt] \footnotesize{(0.1362, 0.1407)}} & \makecell{\small{0.14}\\[-5pt] \footnotesize{(0.1376, 0.1424)}} \\
        \midrule
        \multirow{3}[2]{*}{12}
            & Subgraphs & \makecell{\small{0.7086}\\[-5pt] \footnotesize{(0.702, 0.7153)}} & \makecell{\small{0.9747}\\[-5pt] \footnotesize{(0.9743, 0.9752)}} & \makecell{\small{0.1442}\\[-5pt] \footnotesize{(0.1426, 0.1458)}} & \makecell{\small{0.1119}\\[-5pt] \footnotesize{(0.1104, 0.1134)}} & \makecell{\small{0.1235}\\[-5pt] \footnotesize{(0.1209, 0.1261)}} \\
            & MAML  & \makecell{\small{0.7795}\\[-5pt] \footnotesize{(0.7732, 0.7857)}} & \makecell{\small{0.97}\\[-5pt] \footnotesize{(0.9696, 0.9703)}} & \makecell{\small{0.1307}\\[-5pt] \footnotesize{(0.1295, 0.132)}} & \makecell{\small{0.0751}\\[-5pt] \footnotesize{(0.0743, 0.0758)}} & \makecell{\small{0.0958}\\[-5pt] \footnotesize{(0.0935, 0.0981)}} \\
            & ProtoMAML & \makecell{\small{0.7088}\\[-5pt] \footnotesize{(0.7042, 0.7135)}} & \makecell{\small{0.9822}\\[-5pt] \footnotesize{(0.9819, 0.9824)}} & \makecell{\small{0.1518}\\[-5pt] \footnotesize{(0.1504, 0.1531)}} & \makecell{\small{0.1386}\\[-5pt] \footnotesize{(0.1365, 0.1408)}} & \makecell{\small{0.1464}\\[-5pt] \footnotesize{(0.1444, 0.1483)}} \\
        \midrule
        \multirow{3}[2]{*}{16}
            & Subgraphs & \makecell{\small{0.7136}\\[-5pt] \footnotesize{(0.7072, 0.7199)}} & \makecell{\small{0.9766}\\[-5pt] \footnotesize{(0.9762, 0.9769)}} & \makecell{\small{0.1333}\\[-5pt] \footnotesize{(0.1318, 0.1348)}} & \makecell{\small{0.1025}\\[-5pt] \footnotesize{(0.1011, 0.1038)}} & \makecell{\small{0.1191}\\[-5pt] \footnotesize{(0.1168, 0.1215)}} \\
            & MAML  & \makecell{\small{0.8095}\\[-5pt] \footnotesize{(0.8062, 0.8128)}} & \makecell{\small{0.9789}\\[-5pt] \footnotesize{(0.9787, 0.9792)}} & \makecell{\small{0.1415}\\[-5pt] \footnotesize{(0.1405, 0.1426)}} & \makecell{\small{0.0797}\\[-5pt] \footnotesize{(0.0791, 0.0804)}} & \makecell{\small{0.1168}\\[-5pt] \footnotesize{(0.1151, 0.1185)}} \\
            & ProtoMAML & \makecell{\small{0.7112}\\[-5pt] \footnotesize{(0.7068, 0.7156)}} & \makecell{\small{0.9836}\\[-5pt] \footnotesize{(0.9834, 0.9838)}} & \makecell{\small{0.1392}\\[-5pt] \footnotesize{(0.1379, 0.1404)}} & \makecell{\small{0.1389}\\[-5pt] \footnotesize{(0.1365, 0.1413)}} & \makecell{\small{0.1363}\\[-5pt] \footnotesize{(0.1343, 0.1383)}} \\
        \bottomrule
    \end{tabular}%
    \caption{Transfer of MLP models trained with user-based sampling.}
    \label{tab:coaid_mlp_transfer}%
\end{table*}%


==> tables/main_dataset_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Dataset Stats'
\begin{tabular}{c@{\hspace{0.1\tabcolsep}}c@{\hspace{0.1\tabcolsep}}c@{\hspace{0.1\tabcolsep}}c@{\hspace{0.1\tabcolsep}}}
    \toprule
    \textbf{Dataset} & \textbf{GossipCop} & \textbf{CoAID} & \textbf{TwitterHateSpeech} \\
    \midrule
    \textbf{Task} & \small{Rumour} & \small{Fake News} & \small{Hate Speech} \\[-2pt]
    \textbf{Task} & \small{Celebrity Gossip} & \small{COVID-19} & \small{Entertainment} \\[-2pt]
    
        % Table, inside of a table
        \begin{tabular}{c@{\hspace{0.25\tabcolsep}}c@{\hspace{0.25\tabcolsep}}}
             \small{True} & \small{Fake} \\[-5pt]
             \scriptsize{77.12\%} & \scriptsize{22.88\%}
        \end{tabular} &
        \begin{tabular}{c@{\hspace{0.25\tabcolsep}}c@{\hspace{0.25\tabcolsep}}}
             \small{True} & \small{Fake} \\[-5pt]
             \scriptsize{94.72\%} & \scriptsize{5.28\%}
        \end{tabular} & 
        \begin{tabular}{c@{\hspace{0.25\tabcolsep}}c@{\hspace{0.25\tabcolsep}}c@{\hspace{0.25\tabcolsep}}}
             \small{Racism} & \small{Sexism} & \small{None} \\[-5pt]
             \scriptsize{11.97\%} & \scriptsize{19.43\%} & \scriptsize{68.60\%}
        \end{tabular}
    \\[-2pt]
    \small{Retweet} & \small{Retweet} & \small{Authorship} \\[-2pt]
    
    \midrule
    \footnotesize{17617} & \footnotesize{947} & \footnotesize{16201} \\[-2pt]
    \footnotesize{29229} & \footnotesize{4059} & \footnotesize{1875} \\[-2pt]
    \footnotesize{2334554} & \footnotesize{61254} & \footnotesize{65600} \\[-2pt]
    \bottomrule
\end{tabular}


==> tables/protomaml_transfer_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% \\makecell\{(\\small\{[0-9]\.[0-9]{4}\})\\\\\[-5pt\] \\scriptsize\{\([0-9]\.[0-9]{4}, [0-9]\.[0-9]{4}\)\}\}
\begin{table*}[t]
  \centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
        %\cmidrule(l{4pt}r{4pt}){1-4}\cmidrule(l{4pt}r{4pt}){6-10}
        \toprule
        \multirow{3}{*}{\textbf{k}} & \multicolumn{4}{c}{\textbf{CoAID}} & \multicolumn{5}{c}{\textbf{TwitterHateSpeech}} \\
        
        & \multicolumn{2}{c}{\textbf{F1}} & \multirow{2}{*}{\textbf{MCC}} & \multirow{2}{*}{\makecell{\textbf{Reset} \\ \textbf{MCC}}} 
        & \multicolumn{3}{c}{\textbf{F1}} & \multirow{2}{*}{\textbf{MCC}} & \multirow{2}{*}{\makecell{\textbf{Reset} \\ \textbf{MCC}}} \\
        \cmidrule(l{4pt}r{6pt}){2-3}%\cmidrule(l{4pt}r{8pt}){3-4}
        \cmidrule(l{6pt}r{4pt}){6-8}%\cmidrule(l{4pt}r{4pt}){8-9}
        & Real  & Fake  & &  & Racist & Sexist & None  & &  \\
        \cmidrule(l{4pt}r{8pt}){1-5}\cmidrule(l{8pt}r{4pt}){6-10}
            4 & \small{0.7867} & \small{0.1767} & \small{0.1383} & \small{0.1191} & \small{0.1763} & \small{0.2181} & \small{0.3585} & \small{0.0607} & \small{0.0767} \\
            
            8 & \small{0.8300} & \small{0.1799} & \small{0.1709} & \small{0.1398} & \small{0.1934} & \small{0.2148} & \small{0.3530} & \small{0.0699} & \small{0.0868} \\
            
            12 & \small{0.8331} & \small{0.1675} & \small{0.1689} & \small{0.1304} & \small{0.2545} & \small{0.2554} & \small{0.3503} & \small{0.1109} & \small{0.1025} \\
            
            16 & \small{0.8323} & \small{0.1530} & \small{0.1646} & \small{0.1212} & \small{0.3021} & \small{0.3077} & \small{0.3163} & \small{0.1354} & \small{0.1052} \\
        \bottomrule    
    \end{tabular}
    %}
    \caption{F1 and MCC scores achieved by \textsc{protomaml} during transfer to the auxiliary datasets. Brackets give the 90\% confidence interval. For MCC, a comparison is made to \textsc{protomaml-reset}. This table is presented in more detail in Appendices \ref{appendix:twitter_transfer} and \ref{}}
    \label{tab:addlabel}%
\end{table*}

==> tables/twitter_mlp_ubs_transfer.tex <==
% Table generated by Excel2LaTeX from sheet 'Transfer CoAID - High Adapt'
\begin{landscape}
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{angle=0, width=1.5\textheight}
    \begin{tabular}{clccccccc}
        \toprule
        \multirow{2}[4]{*}{\textbf{k}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Racism}} & \multicolumn{2}{c}{\textbf{Sexism}} & \multicolumn{2}{c}{\textbf{None}} & \textbf{Aggregate} \\
        \cmidrule(l{4pt}r{4pt}){3-4} \cmidrule(l{4pt}r{4pt}){5-6} \cmidrule(l{4pt}r{4pt}){7-8} \cmidrule(l{4pt}r{4pt}){9-9}
        &       & \textbf{F1} & \textbf{AUPR} & \textbf{F1} & \textbf{AUPR} & \textbf{F1} & \textbf{AUPR} & \textbf{MCC} \\
        \midrule
        \multirow{4}[2]{*}{4}
            & Subgraphs & \makecell{\small{0.2091}\\[-5pt] \footnotesize{(0.2042, 0.214)}} & \makecell{\small{0.1647}\\[-5pt] \footnotesize{(0.1627, 0.1666)}} & \makecell{\small{0.225}\\[-5pt] \footnotesize{(0.2214, 0.2286)}} & \makecell{\small{0.1983}\\[-5pt] \footnotesize{(0.1976, 0.199)}} & \makecell{\small{0.4381}\\[-5pt] \footnotesize{(0.4284, 0.4478)}} & \makecell{\small{0.719}\\[-5pt] \footnotesize{(0.7164, 0.7216)}} & \makecell{\small{0.0522}\\[-5pt] \footnotesize{(0.049, 0.0553)}} \\
            & MAML - LH & \makecell{\small{0.1774}\\[-5pt] \footnotesize{(0.1708, 0.1841)}} & \makecell{\small{0.1849}\\[-5pt] \footnotesize{(0.1823, 0.1876)}} & \makecell{\small{0.2447}\\[-5pt] \footnotesize{(0.2415, 0.248)}} & \makecell{\small{0.1962}\\[-5pt] \footnotesize{(0.1951, 0.1973)}} & \makecell{\small{0.4887}\\[-5pt] \footnotesize{(0.4773, 0.5)}} & \makecell{\small{0.7459}\\[-5pt] \footnotesize{(0.7423, 0.7495)}} & \makecell{\small{0.0761}\\[-5pt] \footnotesize{(0.0716, 0.0806)}} \\
            & ProtoMAML & \makecell{\small{0.2549}\\[-5pt] \footnotesize{(0.2517, 0.2581)}} & \makecell{\small{0.1843}\\[-5pt] \footnotesize{(0.1819, 0.1866)}} & \makecell{\small{0.2383}\\[-5pt] \footnotesize{(0.2356, 0.241)}} & \makecell{\small{0.2006}\\[-5pt] \footnotesize{(0.1996, 0.2016)}} & \makecell{\small{0.4604}\\[-5pt] \footnotesize{(0.4545, 0.4662)}} & \makecell{\small{0.7407}\\[-5pt] \footnotesize{(0.7384, 0.7431)}} & \makecell{\small{0.0765}\\[-5pt] \footnotesize{(0.0738, 0.0791)}} \\
        \midrule
        \multirow{4}[2]{*}{8}
            & Subgraphs & \makecell{\small{0.254}\\[-5pt] \footnotesize{(0.2495, 0.2585)}} & \makecell{\small{0.1943}\\[-5pt] \footnotesize{(0.1931, 0.1955)}} & \makecell{\small{0.1979}\\[-5pt] \footnotesize{(0.1934, 0.2024)}} & \makecell{\small{0.2028}\\[-5pt] \footnotesize{(0.202, 0.2037)}} & \makecell{\small{0.5134}\\[-5pt] \footnotesize{(0.5049, 0.5219)}} & \makecell{\small{0.75}\\[-5pt] \footnotesize{(0.748, 0.7521)}} & \makecell{\small{0.0973}\\[-5pt] \footnotesize{(0.0948, 0.0999)}} \\
            & MAML - LH & \makecell{\small{0.213}\\[-5pt] \footnotesize{(0.2066, 0.2194)}} & \makecell{\small{0.2135}\\[-5pt] \footnotesize{(0.2118, 0.2153)}} & \makecell{\small{0.1982}\\[-5pt] \footnotesize{(0.1932, 0.2031)}} & \makecell{\small{0.2014}\\[-5pt] \footnotesize{(0.2003, 0.2025)}} & \makecell{\small{0.6281}\\[-5pt] \footnotesize{(0.6204, 0.6357)}} & \makecell{\small{0.7802}\\[-5pt] \footnotesize{(0.7777, 0.7827)}} & \makecell{\small{0.1235}\\[-5pt] \footnotesize{(0.1199, 0.1271)}} \\
            & ProtoMAML & \makecell{\small{0.2647}\\[-5pt] \footnotesize{(0.2618, 0.2676)}} & \makecell{\small{0.1942}\\[-5pt] \footnotesize{(0.1919, 0.1965)}} & \makecell{\small{0.2339}\\[-5pt] \footnotesize{(0.2312, 0.2365)}} & \makecell{\small{0.2036}\\[-5pt] \footnotesize{(0.2026, 0.2047)}} & \makecell{\small{0.4881}\\[-5pt] \footnotesize{(0.4821, 0.4942)}} & \makecell{\small{0.7495}\\[-5pt] \footnotesize{(0.7474, 0.7517)}} & \makecell{\small{0.0909}\\[-5pt] \footnotesize{(0.0883, 0.0934)}} \\
        \midrule
        \multirow{4}[2]{*}{12}
            & Subgraphs & \makecell{\small{0.2788}\\[-5pt] \footnotesize{(0.2762, 0.2813)}} & \makecell{\small{0.2002}\\[-5pt] \footnotesize{(0.1987, 0.2016)}} & \makecell{\small{0.1835}\\[-5pt] \footnotesize{(0.1788, 0.1882)}} & \makecell{\small{0.1981}\\[-5pt] \footnotesize{(0.1974, 0.1988)}} & \makecell{\small{0.4969}\\[-5pt] \footnotesize{(0.4875, 0.5064)}} & \makecell{\small{0.7488}\\[-5pt] \footnotesize{(0.7467, 0.7509)}} & \makecell{\small{0.0981}\\[-5pt] \footnotesize{(0.0957, 0.1004)}} \\
            & MAML - LH & \makecell{\small{0.3131}\\[-5pt] \footnotesize{(0.3106, 0.3156)}} & \makecell{\small{0.2353}\\[-5pt] \footnotesize{(0.2339, 0.2367)}} & \makecell{\small{0.1934}\\[-5pt] \footnotesize{(0.1886, 0.1982)}} & \makecell{\small{0.2019}\\[-5pt] \footnotesize{(0.2008, 0.203)}} & \makecell{\small{0.5924}\\[-5pt] \footnotesize{(0.5823, 0.6025)}} & \makecell{\small{0.7827}\\[-5pt] \footnotesize{(0.7806, 0.7849)}} & \makecell{\small{0.143}\\[-5pt] \footnotesize{(0.1403, 0.1457)}} \\
            & ProtoMAML & \makecell{\small{0.3064}\\[-5pt] \footnotesize{(0.3041, 0.3087)}} & \makecell{\small{0.2261}\\[-5pt] \footnotesize{(0.224, 0.2281)}} & \makecell{\small{0.2351}\\[-5pt] \footnotesize{(0.2325, 0.2376)}} & \makecell{\small{0.2033}\\[-5pt] \footnotesize{(0.2022, 0.2043)}} & \makecell{\small{0.4957}\\[-5pt] \footnotesize{(0.489, 0.5023)}} & \makecell{\small{0.7577}\\[-5pt] \footnotesize{(0.7557, 0.7596)}} & \makecell{\small{0.1132}\\[-5pt] \footnotesize{(0.111, 0.1154)}} \\
        \midrule
        \multirow{4}[2]{*}{16}
            & Subgraphs & \makecell{\small{0.2937}\\[-5pt] \footnotesize{(0.2917, 0.2958)}} & \makecell{\small{0.2095}\\[-5pt] \footnotesize{(0.2084, 0.2105)}} & \makecell{\small{0.1676}\\[-5pt] \footnotesize{(0.163, 0.1722)}} & \makecell{\small{0.1974}\\[-5pt] \footnotesize{(0.1967, 0.1981)}} & \makecell{\small{0.5119}\\[-5pt] \footnotesize{(0.5028, 0.5211)}} & \makecell{\small{0.7596}\\[-5pt] \footnotesize{(0.7579, 0.7613)}} & \makecell{\small{0.1079}\\[-5pt] \footnotesize{(0.1059, 0.1099)}} \\
            & MAML - LH & \makecell{\small{0.3277}\\[-5pt] \footnotesize{(0.3258, 0.3297)}} & \makecell{\small{0.238}\\[-5pt] \footnotesize{(0.2369, 0.2391)}} & \makecell{\small{0.1764}\\[-5pt] \footnotesize{(0.1717, 0.1811)}} & \makecell{\small{0.2034}\\[-5pt] \footnotesize{(0.2023, 0.2045)}} & \makecell{\small{0.6219}\\[-5pt] \footnotesize{(0.6129, 0.6308)}} & \makecell{\small{0.7886}\\[-5pt] \footnotesize{(0.7869, 0.7904)}} & \makecell{\small{0.156}\\[-5pt] \footnotesize{(0.1539, 0.1582)}} \\
            & ProtoMAML & \makecell{\small{0.3163}\\[-5pt] \footnotesize{(0.3144, 0.3182)}} & \makecell{\small{0.2362}\\[-5pt] \footnotesize{(0.2345, 0.2378)}} & \makecell{\small{0.2244}\\[-5pt] \footnotesize{(0.2218, 0.2271)}} & \makecell{\small{0.2022}\\[-5pt] \footnotesize{(0.2012, 0.2032)}} & \makecell{\small{0.5109}\\[-5pt] \footnotesize{(0.5043, 0.5174)}} & \makecell{\small{0.7647}\\[-5pt] \footnotesize{(0.763, 0.7664)}} & \makecell{\small{0.1216}\\[-5pt] \footnotesize{(0.1196, 0.1236)}} \\
        \bottomrule
    \end{tabular}%
    \end{adjustbox}
    \caption{Add caption}
    \label{tab:addlabel}%
\end{table}
\end{landscape}

==> tables/ubs_query_sampling_statistics.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{clccccc}
        \toprule
        \multirow{2}[2]{*}{\textbf{Dataset}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Metric}}} & \multicolumn{5}{c}{\textbf{Query}} \\[-2pt]
        \cmidrule(l{4pt}r{4pt}){3-7}  
            &       & Mean  & Std. Dev. & Q25   & Median & Q75 \\
        \midrule
        \multirow{7}[-2]{*}{\begin{sideways}GossipCop\end{sideways}}
            & \small{\#Nodes} & \footnotesize{3046.03} & \footnotesize{2821.88} & \footnotesize{609.75} & \footnotesize{2697.5} & \footnotesize{4779.25} \\[-2pt]
            & \small{\#Edges} & \footnotesize{75547.65} & \footnotesize{187261.29} & \footnotesize{5549} & \footnotesize{18839} & \footnotesize{48589} \\[-2pt]
            & \small{\#Docs.} & \footnotesize{2181.1} & \footnotesize{1976.14} & \footnotesize{281} & \footnotesize{1616} & \footnotesize{4108.5} \\[-2pt]
            & \small{Density} & \footnotesize{0.04} & \footnotesize{0.09} & \footnotesize{0} & \footnotesize{0.01} & \footnotesize{0.04} \\[-2pt]
            & \small{Prop. Docs.} & \footnotesize{68.76\%} & \footnotesize{31.75\%} & \footnotesize{43.82\%} & \footnotesize{85.18\%} & \footnotesize{94.75\%} \\[-2pt]
            & \small{Deg. Cent.} & \footnotesize{4.32E-04} & \footnotesize{8.01E-04} & \footnotesize{1.32E-04} & \footnotesize{2.37E-04} & \footnotesize{4.48E-04} \\[-2pt]
            & \small{Eigen Cent.} & \footnotesize{1.50E-04} & \footnotesize{3.78E-04} & \footnotesize{2.66E-05} & \footnotesize{6.56E-05} & \footnotesize{1.40E-04} \\[-2pt]
        \midrule
        \multirow{7}[-2]{*}{\begin{sideways}CoAID\end{sideways}}
            & \small{\#Nodes} & \footnotesize{48.07} & \footnotesize{94.01} & \footnotesize{7} & \footnotesize{18} & \footnotesize{44} \\[-2pt]
            & \small{\#Edges} & \footnotesize{525.98} & \footnotesize{1717.85} & \footnotesize{24} & \footnotesize{80.5} & \footnotesize{257.75} \\[-2pt]
            & \small{\#Docs.} & \footnotesize{1.86} & \footnotesize{1.58} & \footnotesize{1} & \footnotesize{1} & \footnotesize{2} \\[-2pt]
            & \small{Density} & \footnotesize{0.74} & \footnotesize{0.6} & \footnotesize{0.27} & \footnotesize{0.56} & \footnotesize{1.07} \\[-2pt]
            & \small{Prop. Docs.} & \footnotesize{13.93\%} & \footnotesize{14.36\%} & \footnotesize{2.93\%} & \footnotesize{8.33\%} & \footnotesize{20.00\%} \\[-2pt]
            & \small{Deg. Cent.} & \footnotesize{1.67E-03} & \footnotesize{2.73E-03} & \footnotesize{6.02E-04} & \footnotesize{8.02E-04} & \footnotesize{1.60E-03} \\[-2pt]
            & \small{Eigen Cent.} & \footnotesize{5.47E-04} & \footnotesize{4.44E-03} & \footnotesize{1.44E-05} & \footnotesize{4.83E-05} & \footnotesize{1.32E-04} \\[-2pt]
        \midrule
        \multirow{7}[-2]{*}{\begin{sideways}TwitterHS\end{sideways}}
            & \small{\#Nodes} & \footnotesize{1485.73} & \footnotesize{1009.45} & \footnotesize{220} & \footnotesize{2056} & \footnotesize{2571} \\[-2pt]
            & \small{\#Edges} & \footnotesize{4511.72} & \footnotesize{2967.31} & \footnotesize{1774} & \footnotesize{6168} & \footnotesize{7711} \\[-2pt]
            & \small{\#Docs.} & \footnotesize{1476.97} & \footnotesize{1017.5} & \footnotesize{22} & \footnotesize{2053} & \footnotesize{2569} \\[-2pt]
            & \small{Density} & \footnotesize{0.23} & \footnotesize{0.49} & \footnotesize{0} & \footnotesize{0} & \footnotesize{0.13} \\[-2pt]
            & \small{Prop. Docs.} & \footnotesize{81.80\%} & \footnotesize{32.20\%} & \footnotesize{81.25\%} & \footnotesize{99.85\%} & \footnotesize{99.92\%} \\[-2pt]
            & \small{Deg. Cent.} & \footnotesize{2.97E-04} & \footnotesize{1.08E-19} & \footnotesize{2.97E-04} & \footnotesize{2.97E-04} & \footnotesize{2.97E-04} \\[-2pt]
            & \small{Eigen Cent.} & \footnotesize{4.12E-03} & \footnotesize{6.36E-03} & \footnotesize{7.01E-08} & \footnotesize{3.70E-07} & \footnotesize{1.39E-02} \\[-2pt]
        \bottomrule
    \end{tabular}%
    \caption{Same as Table \ref{tab:ubs_support_stats}, but now for the query graphs.}
    \label{tab:ubs_query_stats}
\end{table*}

